Vibe Spaces for Creatively Connecting and Expressing Visual Concepts

Creating new visual concepts often requires connecting distinct ideas through their most relevant shared attributes -- their vibe. We introduce Vibe Blending, a novel task for generating coherent and meaningful hybrids that reveals these shared attributes between images. Achieving such blends is challenging for current methods, which struggle to identify and traverse nonlinear paths linking distant concepts in latent space. We propose Vibe Space, a hierarchical graph manifold that learns low-dimensional geodesics in feature spaces like CLIP, enabling smooth and semantically consistent transitions between concepts. To evaluate creative quality, we design a cognitively inspired framework combining human judgments, LLM reasoning, and a geometric path-based difficulty score. We find that Vibe Space produces blends that humans consistently rate as more creative and coherent than current methods.

==> figures/analogy_qualitative.tex <==
\begin{figure*}[!th]
    \centering
    \includegraphics[trim=0in 0in 0in 0in, clip,width=\textwidth]{figures/analogy_qualitative.jpg}
    \caption{}
\label{fig:analogy_qualitative}
\end{figure*}


==> figures/claim2.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[trim=0in 0in 0in 0in, clip,width=\textwidth]{figures/claim2.jpg}
    \vspace{-20 pt}
    \caption{
    }
    
    \label{fig:claim2}
\end{figure*}



==> figures/n_image_blending.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/n_image_blending.jpg}
    \caption{\todo{\andrew{}} }
\label{fig:n_image_blending}
\end{figure}

==> figures/small1.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/small1.jpg}
    \caption{Examples of semantic correspondence matching.}
    \label{fig:placeholder}
\end{figure}

==> figures/small2.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{small2.jpg}
    \caption{...}
    \label{fig:placeholder}
\end{figure}
